Heterogeneity in demand and optimal price conditioning for local rail transport

This paper describes the results of research project on optimal pricing for LLC "Perm Local Rail Company". In this study we propose a regression tree based approach for estimation of demand function for local rail tickets considering high degree of demand heterogeneity by various trip directions and the goals of travel. Employing detailed data on ticket sales for 5 years we estimate the parameters of demand function and reveal the significant variation in price elasticity of demand. While in average the demand is elastic by price, near a quarter of trips is characterized by weakly elastic demand. Lower elasticity of demand is correlated with lower degree of competition with other transport and inflexible frequency of travel.

==> Sections/0_Title_page.tex <==
\title{Heterogeneity in demand and optimal price conditioning for local rail transport}
%
\titlerunning{Demand for rail}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here
%
\author{Evgeniy M. Ozhegov\inst{1} \and Alina M. Ozhegova\inst{2}   
 }
%
\authorrunning{Ozhegov, Ozhegova}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{National Research University Higher School of Economics.\\Research Group for Applied Markets and Enterprises Studies, Research fellow. 
\email{tos600@gmail.com}\\ \and
National Research University Higher School of Economics.\\Research Group for Applied Markets and Enterprises Studies, Junior research fellow.\\
\email{arbuzanakova@gmail.com}}
\maketitle             

%
%
\section*{Abstract}

This paper describes the results of research project on optimal pricing for LLC «Perm Local Rail Company». In this study we propose a regression tree based approach for estimation of demand function for local rail tickets considering high degree of demand heterogeneity by various trip directions and the goals of travel. Employing detailed data on ticket sales for 5 years we estimate the parameters of demand function and reveal the significant variation in price elasticity of demand. While in average the demand is elastic by price, near a quarter of trips is characterized by weakly elastic demand. Lower elasticity of demand is correlated with lower degree of competition with other transport and inflexible frequency of travel. \\

\noindent \textbf{Keywords:} demand, rail transport, heterogeneity, price elasticity, optimal pricing.\\

\noindent \textbf{JEL classification:} D12, L92, R41.
